Automatic Synthesis of Parallel Unix Commands and Pipelines with KumQuat

We present KumQuat, a system for automatically generating data parallel implementations of Unix shell commands and pipelines. The generated parallel versions split input streams, execute multiple instantiations of the original pipeline commands to process the splits in parallel, then combine the resulting parallel outputs to produce the final output stream. KumQuat automatically synthesizes the combine operators, with a domain-specific combiner language acting as a strong regularizer that promotes efficient inference of correct combiners. We evaluate KumQuat on 70 benchmark scripts that together have a total of 427 stages. KumQuat synthesizes a correct combiner for 113 of the 121 unique commands that appear in these benchmark scripts. The synthesis times vary between 39 seconds and 331 seconds with a median of 60 seconds. We present experimental results that show that these combiners enable the effective parallelization of our benchmark scripts.

==> conclusion.tex <==
\section{Conclusion}
\label{discussion}
This paper presented \sys, a system for automatically synthesizing parallel and distributed versions of \unix commands.
\sys decomposes commands into two phases:
  (i) a parallel mapper that applies the original command to produce partial results, and 
  (ii) an combiner that combines the partial results and is synthesized by \sys.
To synthesize the combiner, \sys applies program inference on the command---with a key insight being that the parallel specification to be inferred is the already-available sequential command.
\sys synthesizes the merger by applying repeated rounds of exploration;
  at each round, it compares the results of the synthesized program with those from the sequential program to discard invalid candidates.
\sys's implementation supports two back-ends.
A parallel back-end accelerates execution on a single host without any additional runtime support.
A distributed back-end offers program- and data-transformation wrappers to bolt \sys's two phases on Hadoop, offloading several distributed-systems challenges to a production-grade distributed computing runtime.
\sys can offer significant parallel speedups and synthesizes combiners for most of our benchmark commands within a minute. 
\vfill

